Adapting Large Language Models for Content Moderation: Pitfalls in Data Engineering and Supervised Fine-tuning

Nowadays, billions of people engage in communication and express their opinions on the internet daily. Unfortunately, not all of these expressions are friendly or compliant, making content moderation an indispensable task. A common approach is to use a discriminative model to classify the content, but this method often requires strict data engineering, otherwise it will face unacceptable overfitting. With the successful development of Large Language Models (LLMs) in recent years, LLM-based methods have become a feasible solution for handling tasks in various domains. Thanks to the knowledge of the foundation models, we can develop more robust privately deployed models with limited data via fine-tuning these foundation models. Moreover, as a generative model, it can provide detailed analysis of the review process, enhancing interpretability. In this paper, we introduce how to fine-tune a LLM model that can be privately deployed for content moderation. Specifically, we discuss the differences between discriminative and generative models using content moderation as an example. Additionally, we reveal that incorporating reasoning processes during the fine-tuning of LLMs can effectively alleviate overfitting, even if the model is not allowed to directly output reasoning processes during deployment. We present a complete process, from data collection and construction to model training and overfitting elimination, for fine-tuning LLMs in vertical domain deployments. We report the entire research process and the key findings in this paper, hoping to provide valuable experience for researchers who are fine-tuning privately deployed models in their domain-specific research.

==> sections/intro.tex <==
Content moderation serves as a crucial role aiming to filter detrimental content on the Internet, including offensive, pornographic, or violent descriptions~\citep{dinan2019build,jahan2023systematic}. The most natural approach entails generating a distributionally analogous training dataset based on a given task objective, and subsequently utilizing the dataset to train a classification network~\citep{deng2022cold,husain2021survey}. Nevertheless, this method proves to be impractical in real-world applications due to its inadequate robustness, and researchers encounter challenges in overcoming model overfitting~\citep{djandji2020multi,anand2023deep}. Moreover, it lacks interpretability, complicating the process of elucidating the rationale behind the model's decisions and pinpointing the pseudo-associations that result in incorrect classifications. Although certain methods strive to explicate the basis for the model's decisions, such as scrutinizing the network's activation states to discern the origins of erroneous predictions~\citep{patro2019u,jung2021towards} and employing model editing to rectify the model~\citep{meng2022locating}, these approaches are unwieldy for natural language tasks and fail to offer the most intuitive explanations.



% A more intuitive approach is to demonstrate the moderation process for each sample, allowing for a clear explanation of the classification basis. Some current large language models (LLMs), such as GPT-4, have already achieved promising performance. However, using such services for large-scale, continuous content moderation is unrealistic due to the high costs and potential privacy concerns. Therefore, a more practical approach is to deploy a relatively smaller language model locally to accomplish the task. Unfortunately, compared to GPT-4, current open-source small models have not undergone sufficient strong supervised fine-tuning (SFT) and reinforcement learning from human feedback (RLHF), leading to subpar performance on domain-specific tasks. A natural solution is to create a training dataset with annotated analysis processes to fine-tune the open-source LLMs for the target task. However, this method has two issues: the inconsistency in language style and cognitive standards among different annotators, and the high cost of annotation. Consequently, obtaining high-quality annotated data automatically becomes a problem that needs to be addressed.

Recently, OpenAI introduce a novel strategy for content moderation that leverages the capabilities of GPT-4~\citep{openai2023gpt4}. Specifically, policy experts formulate a comprehensive content policy and annotate a select set of examples to create a ``golden dataset." Subsequently, GPT-4 is instructed to read this content policy, label the same dataset, and reconcile any discrepancies between its own judgments and those made by human experts. This iterative methodology involves intricate analysis of ambiguous policy language and offers subsequent clarifications as required, continuing until the desired level of policy quality is achieved~\citep{lilian2023moderation}. For practical business applications, the implementation of a privately deployed model is imperative, particularly to address policy-related issues such as user privacy~\citep{scheffler2023sok}. Current open-source LLMs~\citep{du2022glm,zeng2022glm} have not been subjected to adequate Supervised Fine-Tuning (SFT) or Reinforcement Learning from Human Feedback (RLHF), resulting in less-than-optimal performance in domain-specific tasks. To address this issue, some studies have explored the fine-tuning of LLMs as classifiers~\citep{aws}. However, we observe that such fine-tuning often leads to severe overfitting, making these models unsuitable for deployment in open environments. In the realm of mathematical task analysis, various papers demonstrate the efficacy of incorporating a Chain-of-Thought (CoT) paradigm to enhance model performance~\citep{imani2023mathprompter,gao2023pal}. OpenAI's recent research also unveiles a step-by-step verification strategy during the fine-tuning phase to tackle complex mathematical tasks~\citep{lightman2023lets}. These methodologies collectively highlight that the inclusion of a reasoning process prior to generating a final answer can significantly improve a model's generalization capabilities. Inspired by these works, a question is raised: What impact would the addition of a reasoning process have on the fine-tuning of LLMs for content moderation? To explore this, we employ CoT during fine-tuning LLMs, prompting the model to undertake analytical steps and identify harmful content before proceeding to classification. The framework for this is illustrated in Fig.~\ref{fig:cover}. Specifically, we leverage a more powerful LLM API service, such as ChatGPT, to generate CoT in the training set and subsequently train a privately deploys model using this augmented dataset. Notably, aside from enhancing the model's generalization capability, we found that the more powerful LLM also generated a significant volume of erroneous response, which we address according to different approaches and report the findings accordingly.







% However, this method has two issues: the inconsistency in language style and cognitive standards among different annotators, and the high cost of annotation. Consequently, obtaining high-quality annotated data automatically becomes a problem that needs to be addressed. 

% Leveraging more powerful models to generate thought chains is a feasible approach, as these models possess greater capabilities and can often generate high-quality thought chains without incurring excessive costs. However, this strategy still faces several challenges in practice: (1) even powerful models like may misclassify some samples, and (2) the analysis process for some samples may not be consistent with the classification results, such as when a sample is classified into the correct category but the analysis process description leans more towards another category.


% In this paper, we present an automated approach to effectively address the challenges arising from the misleading nature of large models. Our proposed method focuses on dynamically acquiring high-quality training data to fine-tune smaller models. Specifically, we employ two key strategies:

% (1) we utilize consistency testing to evaluate the "classification results" of model-generated responses against the actual labels. This enables us to identify and filter out responses of lower quality. We subsequently perform model self-reflection on these low-quality responses, updating the answers accordingly. This iterative process involves repeating consistency testing after each update to eliminate any remaining incorrect samples.
% (2) we meticulously examine the consistency between the analysis process and the classification results in the response. This step ensures the establishment of a causal relationship between the analysis process and the obtained classification results.

In this paper, we investigate the efficacy of employing cloud LLM services such as ChatGPT to generate CoT during the fine-tuning process of a privately deployed LLM for content moderation. Specifically, we examine whether the CoT generated by the cloud LLM services can augment the training dataset and evaluate the model's capacity for self-recheck in the generated CoT. Our key findings are as follows:
(1) Directly fine-tuning the LLM to function as a classifier results in severe overfitting, making the model ineffective for deployment in open environments.
(2) We can effectively mitigate overfitting by incorporating reasons generated by cloud LLM services such as ChatGPT into the fine-tuning process of the privately deployed model.
(3) If the initial response of ChatGPT is incorrect, its rephrased answer is not suitable to be used as fine-tuning data, even if ChatGPT corrects the classification result in the rephrased response.
(4) The straightforward yet effective approach for improve the quality of training set is to remove the samples in which ChatGPT's responses are incorrect. 
(5) LLMs have an upper bound of capability when it is fine-tuned with Parameter-Efficient Fine-Tuning (PEFT), and complex and detailed reasoning processes may lead to worse performance of certain models due to the difficulties in fitting complex reasoning processes.



